From Hindsight to Foresight: Dissecting Clinical Evidence Acquisition in Large Language Models

Large language models (LLMs) often diagnose full sight, static clinical cases well yet struggle in foresight, dynamic diagnosis. Prior work has improved this limitation by quantifying the information models acquire and by developing stronger follow-up strategies to improve diagnostic accuracy. In contrast, we introduce a distinctive hindsight to systematically dissect why LLMs fail to acquire diagnostically critical evidence, tracing the failure from evidence identification, utilization and downstream diagnostic updating through not only diagnostic accuracy, but also evidence coverage, trajectory dynamics, and elicited probability and information entropy. Starting experiments from the breakdown at the level of capabilities, to the diagnosis of the pre-event state before the evidence arrives, and to the post-event state transition after the evidence arrives, our research has revealed the profound limitations and internal causes existing in the dynamic diagnostic process. At the same time, we have also conducted sufficient verification and generalization experiments to prove that these limitations are widespread. Together, these findings shift the central challenge from whether LLMs possess relevant clinical knowledge to whether they can identify, acquire, and effectively use the right evidence under clinical diagnosis and conduct a more detailed mechanism analysis to identify the exact location of the capability gap.

==> generated/table_clinician_agreement.tex <==
\begin{tabular}{lrr}
\toprule
Archived slot outcome & Exact agreement & Kappa / ICC \\
\midrule
Top-1 relevance & 100.0\% & n.a. \\
Top-3 critical evidence & 100.0\% & n.a. \\
Top-3 order & 90.0\% & 0.000 \\
Missing-evidence flag & 96.0\% & 0.000 \\
Answer-revealing flag & 96.0\% & 0.000 \\
Preferred Top-1 evidence & 88.0\% & -- \\
Preferred Top-3 evidence & 0.810 Jaccard & -- \\
Quality rating & -- & QWK 0.148; ICC 0.150 \\
Confidence rating & -- & QWK 0.000; ICC 0.000 \\
\bottomrule
\end{tabular}


==> generated/table_clinician_audit.tex <==
\begin{tabular}{lrr}
\toprule
Archived review-record outcome & Estimate & 95\% CI \\
\midrule
Top-1 diagnostically relevant & 100.0\% & [100.0\%, 100.0\%] \\
Top-3 contains critical evidence & 100.0\% & [100.0\%, 100.0\%] \\
Top-3 order reasonable (strict) & 97.5\% & [95.5\%, 99.5\%] \\
Critical evidence missing from Top-3 & 1.0\% & [0.0\%, 2.5\%] \\
Any Top-6 item answer-revealing & 1.0\% & [0.0\%, 2.5\%] \\
Reviewer--Hindsight Top-1 agreement & 89.0\% & [83.0\%, 94.5\%] \\
Reviewer--Hindsight Top-3 Jaccard & 0.870 & [0.829, 0.907] \\
Overall selector quality (1--5) & 4.57 & [4.48, 4.66] \\
\bottomrule
\end{tabular}


==> generated/table_critical_fact_rescue.tex <==
% Auto-generated by analyze_critical_fact_rescue.py; do not edit.
\begin{tabular}{lrrl}
\toprule
Condition/contrast & Numerator & N & Estimate (95\% CI) \\
\midrule
S1: add missing Hindsight Top-1 & 19 & 114 & 16.7\% [9.6, 23.7] \\
S2: add random unseen control & 6 & 114 & 5.3\% [1.8, 9.6] \\
Paired S1--S2 & 13 & 114 & 11.4 pp [4.4, 19.3] \\
Worst-case S1 (2 salvages incorrect) & 18 & 114 & 15.8\% [9.6, 22.8] \\
\bottomrule
\end{tabular}


==> generated/table_critical_fact_rescue_sensitivity.tex <==
% Auto-generated by analyze_critical_fact_rescue.py; do not edit.
\begin{tabular}{lrrrl}
\toprule
Subset & S1 correct & S2 correct & N & Paired difference (95\% CI) \\
\midrule
Hindsight Top-1 prefix correct & 18 & 5 & 53 & 24.5 pp [11.3, 37.7] \\
Hindsight Top-1 prefix incorrect & 1 & 1 & 61 & 0.0 pp [-4.9, 4.9] \\
Control modality matched & 12 & 4 & 83 & 9.6 pp [2.4, 18.1] \\
Control fallback modality & 7 & 2 & 31 & 16.1 pp [0.0, 32.3] \\
\bottomrule
\end{tabular}


==> generated/table_evimed.tex <==
\begin{tabular}{lrrrr}
\toprule
Strategy & ICR & Accuracy & Unique facts & No-new rate \\
\midrule
Official baseline & 28.3\% & 23.5\% & 5.74 & 0.0\% \\
Menu control & 32.6\% & 35.0\% & 6.49 & 82.7\% \\
Official REFINE & 46.2\% & 38.0\% & 9.48 & 0.0\% \\
Hindsight reference & 73.3\% & 53.0\% & 14.12 & 0.0\% \\
\bottomrule
\end{tabular}


==> generated/table_matched.tex <==
\begin{tabular}{rrrrrr}
\toprule
Budget & Mean actual facts & Foresight acc. & Matched Hindsight acc. & Gap & 95\% CI \\
\midrule
3 & 2.09 & 33.1\% & 63.0\% & 29.8\% & [22.1\%, 37.6\%] \\
6 & 3.52 & 42.0\% & 70.7\% & 28.7\% & [20.4\%, 37.0\%] \\
\bottomrule
\end{tabular}


==> generated/table_menu.tex <==
\begin{tabular}{rrrrrrr}
\toprule
$k$ & Free acc. & Menu acc. & Hindsight acc. & Free facts & Menu facts & Hindsight facts \\
\midrule
1 & 16.7\% & 25.0\% & 57.5\% & 0.89 & 0.90 & 1.00 \\
2 & 26.7\% & 30.0\% & 70.0\% & 1.57 & 1.40 & 2.00 \\
3 & 31.7\% & 31.7\% & 75.0\% & 2.09 & 1.61 & 3.00 \\
4 & 33.3\% & 38.3\% & 76.7\% & 2.58 & 1.81 & 4.00 \\
5 & 31.7\% & 35.8\% & 78.3\% & 3.05 & 2.02 & 5.00 \\
6 & 38.3\% & 42.5\% & 75.8\% & 3.43 & 2.19 & 6.00 \\
\bottomrule
\end{tabular}


==> generated/table_primary.tex <==
\begin{tabular}{rrrrrr}
\toprule
$k$ & Foresight & Hindsight & Gap & 95\% CI low & 95\% CI high \\
\midrule
1 & 18.8\% & 55.8\% & 37.0\% & 29.3\% & 45.3\% \\
2 & 29.3\% & 66.3\% & 37.0\% & 28.7\% & 45.3\% \\
3 & 33.1\% & 73.5\% & 40.3\% & 32.6\% & 48.6\% \\
4 & 35.9\% & 75.1\% & 39.2\% & 31.5\% & 47.0\% \\
5 & 34.8\% & 74.0\% & 39.2\% & 30.9\% & 47.5\% \\
6 & 42.0\% & 75.7\% & 33.7\% & 26.0\% & 41.4\% \\
\bottomrule
\end{tabular}


==> generated/table_readout.tex <==
\begin{tabular}{lrrrr}
\toprule
Perturbation & Top-1 & $\rho$(gold) & $\rho$(entropy) & Median JSD \\
\midrule
Test-retest & 75.4\% & 0.867 & 0.556 & 0.081 \\
Candidate order & 65.4\% & 0.814 & 0.485 & 0.088 \\
Prompt paraphrase & 66.7\% & 0.680 & 0.479 & 0.093 \\
Candidate-support replacement & 68.3\% & 0.823 & 0.550 & 0.100 \\
\bottomrule
\end{tabular}


==> generated/table_selector.tex <==
\begin{tabular}{llrrrr}
\toprule
Selector & Variant & Top-1 & Jaccard & RBO@6 & Hind@3 \\
\midrule
Gemini & cross selector & 72.5\% & 0.713 & 0.809 & 72.5\% \\
GPT & cross selector & 67.5\% & 0.710 & 0.805 & 73.8\% \\
DS & order 1 & 77.0\% & 0.719 & 0.829 & 70.0\% \\
DS & order 2 & 77.0\% & 0.769 & 0.833 & 70.0\% \\
DS & primary & 100.0\% & 1.000 & 1.000 & 76.0\% \\
DS & prompt alt & 78.0\% & 0.747 & 0.829 & 72.0\% \\
DS & repeat 1 & 79.0\% & 0.769 & 0.854 & 70.0\% \\
DS & repeat 2 & 80.0\% & 0.813 & 0.851 & 71.0\% \\
DS & repeat 3 & 80.0\% & 0.798 & 0.866 & 68.0\% \\
\bottomrule
\end{tabular}


==> generated/table_trajectory_dynamics.tex <==
% Auto-generated by analyze_trajectory_dynamics.py; do not edit.
\begin{tabular}{lrrl}
\toprule
Measure & Numerator & Denominator & Estimate (95\% CI) \\
\midrule
Wrong-state persistence & 572 & 630 & 90.8\% [88.2, 93.1] \\
Wrong-to-correct transition & 58 & 630 & 9.2\% [6.9, 11.8] \\
Correct-state retention & 259 & 275 & 94.2\% [90.9, 96.9] \\
Action stagnation rate & -- & 181 cases & 41.3\% [37.9, 44.8] \\
Failure recovery by next action & 134 & 343 & 39.1\% [33.2, 45.4] \\
ECNR@1 & 15 & 38 & 39.5\% [23.9, 55.6] \\
ECNR@3 & 48 & 91 & 52.7\% [42.4, 62.7] \\
ECNR@6 & 106 & 159 & 66.7\% [58.9, 74.0] \\
\bottomrule
\end{tabular}


==> generated/table_value.tex <==
\begin{tabular}{lrrr}
\toprule
Choice policy & Estimable & Mean CVP & Mean selected TDG \\
\midrule
Actual free & 138 & 0.570 & 2.274 \\
Prospective menu & 147 & 0.565 & 2.750 \\
Random panel & 200 & 0.639 & 2.207 \\
\bottomrule
\end{tabular}


==> generated/table_xmodel.tex <==
\begin{tabular}{lrrrr}
\toprule
Model & Atomic@3 & Hind@3 & Gap & 95\% CI \\
\midrule
DeepSeek V3.2 & 35.6\% & 55.9\% & 20.3\% & [6.8\%, 33.9\%] \\
GPT-5.4 & 47.5\% & 66.1\% & 18.6\% & [10.2\%, 28.8\%] \\
Gemini 3.1 Pro Preview & 54.2\% & 62.7\% & 8.5\% & [-3.4\%, 20.3\%] \\
GLM 5.2 & 37.3\% & 61.0\% & 23.7\% & [11.9\%, 37.3\%] \\
\bottomrule
\end{tabular}


==> tables/results/C/count-matched.tex <==
\begin{table}[t]
    \centering
    \caption{\textbf{Same evidence amount does not eliminate the diagnostic separation.} For every case and budget, Hindsight is truncated to the number of unique evidence items actually obtained by Foresight. Panel A is the prespecified primary cohort; Panel B is a separate fixed continuation cohort and is not pooled with Panel A. Differences are count-matched Hindsight minus Foresight with paired case-level 95\% confidence intervals.}
    \label{tab:matched}
    \begingroup
    \scriptsize
    \setlength{\tabcolsep}{3.3pt}
    \renewcommand{\arraystretch}{0.96}
    \begin{tabular}{@{}lrrrr@{}}
        \toprule
        Budget & Mean evidence & Foresight & Matched Hindsight & Difference [95\% CI] \\
        \midrule
        \multicolumn{5}{@{}l}{\textit{Panel A: prespecified primary cohort ($N=\PrimaryN$)}} \\
        $k=3$ & \MatchedFactsThree{} & \MatchedForesightThree{} & \MatchedDUThree{} & \CPrimaryGapThreeCell{} \\
        $k=6$ & \CPrimaryFactsSix{} & \CPrimaryForesightSix{} & \CPrimaryDUSix{} & \CPrimaryGapSixCell{} \\
        \midrule
        \multicolumn{5}{@{}l}{\textit{Panel B: fixed continuation cohort ($N=\KExtensionN$)}} \\
        $k=6$  & \KFactsSix{}   & \KAtomicSix{}    & \KDUSixMatched{}    & \KMatchedGapSix{}~\KMatchedGapSixCI{} \\
        $k=12$ & \KFactsTwelve{} & \KAtomicTwelve{} & \KDUTwelveMatched{} & \KMatchedGapTwelve{}~\KMatchedGapTwelveCI{} \\
        \bottomrule
    \end{tabular}
    \endgroup
\end{table}


==> tables/results/E/validation-ablation.tex <==
\begin{table}[t]
\centering
\caption{\textbf{Ablation synthesis.} Each control isolates a different alternative explanation using its own prespecified cohort and estimand; effects are therefore not additive. Confidence intervals are paired case-level 95\% intervals where available.}
\label{tab:e-ablation}
\begingroup
\scriptsize
\setlength{\tabcolsep}{3.0pt}
\renewcommand{\arraystretch}{1.03}
\begin{tabularx}{\linewidth}{@{}p{0.19\linewidth}p{0.20\linewidth}p{0.23\linewidth}X@{}}
\toprule
\textbf{Control} & \textbf{Component tested} & \textbf{Observed effect} & \textbf{Supported conclusion} \\
\midrule
Result-blind menu & Free-text target generation & 31.7 vs. 31.7 (+0.0 pp) & Removing free-text generation is insufficient \\
Case-specific count matching & Evidence quantity & +29.8 pp [22.1, 37.6] & Equal quantity leaves a large separation \\
Same-set reranking & Order within the Foresight set & +9.3 pp [5.5, 13.2] & Order contributes, but does not recover the full gap \\
Evidence-set replacement & Evidence identity & +26.7 pp [19.0, 34.5] & Which evidence is present has the larger effect \\
Critical-evidence rescue & Specific value of the added evidence & +11.4 pp [4.4, 19.3] & Missing useful evidence causally contributes \\
\bottomrule
\end{tabularx}
\endgroup
\end{table}


==> tables/setup/core-metrics.tex <==
\begin{table}[H]
\centering
\label{tab:metrics}
\small

\noindent
\begin{minipage}[t]{0.48\linewidth}
\textbf{Diagnostic accuracy}\quad
$\displaystyle
A(k)=\frac{1}{N}\sum_c
\mathbf{1}\!\left[\hat y_c(k)=y_c^\star\right]$
\end{minipage}
\hfill
\begin{minipage}[t]{0.48\linewidth}
\textbf{Evidence yield}\quad
$\displaystyle
F(k)=\frac{1}{N}\sum_c
\frac{|\mathcal{E}_c(k)|}{k}$
\end{minipage}

\par\smallskip

\noindent
\begin{minipage}[t]{0.48\linewidth}
\textbf{Critical-evidence reach}\quad
$\displaystyle
R_M(k)=\frac{1}{N}\sum_c
\frac{|\mathcal{E}_c(k)\cap\mathcal{C}_c^{(M)}|}{M}$
\end{minipage}
\hfill
\begin{minipage}[t]{0.48\linewidth}
\textbf{Information coverage}\quad
$\displaystyle
\mathrm{ICR}(k)=\frac{1}{N}\sum_c
\frac{|\mathcal{E}_c(k)\cap\mathcal{G}_c|}
{|\mathcal{G}_c|}$
\end{minipage}

\par\smallskip

\noindent
\begin{minipage}[t]{0.48\linewidth}
\textbf{Stable sufficiency}\quad
$\displaystyle
S(k)=\frac{1}{N}\sum_c
\mathbf{1}\!\left[k_c^\star\le k\right]$

\vspace{-2pt}
{\footnotesize
$\displaystyle
k_c^\star=\min\{j:\hat y_c(t)=y_c^\star,\ \forall t\ge j\}$}
\end{minipage}
\hfill
\begin{minipage}[t]{0.48\linewidth}
\textbf{Wrong-state persistence}\quad
$\displaystyle
W_{c,k}=\mathbf{1}\!\left[\hat y_c(k)\ne y_c^\star\right]$

\vspace{-2pt}
{\footnotesize
$\displaystyle
\mathrm{WSP}=
\frac{\sum_{c,k}W_{c,k}W_{c,k+1}}
{\sum_{c,k}W_{c,k}}$}
\end{minipage}

\end{table}
